Towards Effective Experiential Learning: Dual Guidance for Utilization and Internalization

Recently, reinforcement learning~(RL) has become an important approach for improving the capabilities of large language models~(LLMs). In particular, reinforcement learning from verifiable rewards~(RLVR) has emerged as a promising paradigm for reasoning tasks. However, existing RL-based training still remains only a rough approximation to human learning. Human learners leverage both external and internal experience to guide exploration and gradually internalize useful trajectories into stable knowledge. Motivated by this gap, we ask: how can LLMs better utilize and internalize experience during RLVR training? To answer this question, we propose \textbf{D}ual \textbf{G}uidance \textbf{O}ptimization~(\textbf{DGO}), a unified framework that leverages \emph{external} and \emph{internal experience} to improve training effectiveness. Specifically, DGO first constructs an experience bank from previously explored trajectories. The policy then performs exploration under the joint guidance of the experience bank and the model's internal knowledge. The resulting trajectories are further used to refine the experience bank and optimize model parameters, forming a closed loop of experience utilization and internalization. Experiments show that DGO consistently outperforms baseline methods, suggesting that better utilization and internalization of experience lead to more effective reasoning.

==> archive/safety_rlhf.tex <==
\subsubsection{Reinforcement Learning for Dynamic Safety Alignment}

This section delineates the use of Reinforcement Learning (RL) for the safety alignment of Code Large Language Models (CLLMs). This paradigm reconceptualizes alignment not as a static, dataset-driven procedure, but as a dynamic optimization problem where the model learns secure coding strategies through iterative trial and error, governed by a reward signal derived from safety-pertinent feedback. By iteratively optimizing its code generation policy based on the consequences of its outputs, the model can move beyond simple pattern matching and develop a more robust understanding of safety principles.

\paragraph{The RLHF/RLAIF Framework for Code Safety}

\begin{itemize}
\item \textbf{Core Mechanism}  
The standard methodology for this alignment process is Reinforcement Learning from Human Feedback (RLHF). This process typically unfolds in three stages. First, a base language model is fine-tuned on a high-quality dataset to create a supervised fine-tuned (SFT) model. Second, a reward model is trained on human preference data, where annotators rank different outputs generated by the SFT model. Finally, this reward model provides a scalar reward signal to the SFT model, which is further fine-tuned using an RL algorithm like Proximal Policy Optimization (PPO) to generate outputs that maximize the reward score, as established in foundational works like ( [Training language models to follow instructions with human feedback] ).
\item \textbf{From RLHF to RLAIF}  
The operational exigencies of large-scale human annotation have necessitated a shift toward automated feedback. Reinforcement Learning from AI Feedback (RLAIF) emerges as a powerful alternative, addressing the cost and scalability limitations of RLHF. As detailed in ( [Constitutional AI: Harmlessness from AI Feedback] ), RLAIF replaces human annotators with a capable ``judge'' LLM or a set of predefined principles---a ``constitution''---to generate preference labels at scale. This is particularly advantageous in the coding domain, where an AI judge can be augmented with deterministic code analysis tools to provide feedback that is both scalable and grounded in verifiable technical criteria, a concept explored in frameworks like ( [ACECODER: Acing Coder RL via Automated Test-Case Synthesis] ).
\end{itemize}

\paragraph{Constructing the Safety Reward Signal}

The efficacy of any RL-based alignment process is fundamentally dependent on the quality of its reward function. A poorly designed reward function can lead to ``reward hacking,'' where the model maximizes the reward metric without achieving the intended safety goal.

\begin{itemize}
\item \textbf{Verifiable Feedback as Reward}  
The most reliable reward signals are derived from verifiable and objective outcomes. For code generation, this includes:
\item \textbf{Execution and Test Results:} A positive reward can be assigned to code that compiles and passes unit tests, while a negative reward is given for failures. This provides a clear measure of functional correctness, a technique leveraged in ( [ACECODER: Acing Coder RL via Automated Test-Case Synthesis] ).
\item \textbf{Static Analysis Tools (SAST):} Outputs from tools like linters and security analyzers can be integrated into the reward function. Code that generates no warnings receives a positive reward, while penalties are applied based on the number and severity of detected vulnerabilities. This approach is central to the ( [CRScore: Reinforcement Learning with Verifiable Tool and AI Feedback for Code Review] ) framework.
\item \textbf{AI-Generated Feedback (RLAIF) as Reward}  
For nuanced safety issues that automated tools may miss, RLAIF provides a scalable method for generating reward signals. A powerful teacher model evaluates the code produced by the student model, and these evaluations are used to train the reward model, as demonstrated in ( [R2Vul: Learning to Reason about Software Vulnerabilities with Reinforcement Learning and Structured Reasoning Distillation] ). This can be combined with Constitutional AI principles, where the reward model is trained to prefer outputs that adhere to safety rules, such as ``the code must not contain hard-coded secrets,'' an idea explored in ( [Constitutional AI: Harmlessness from AI Feedback] ).
\item \textbf{Hybrid Reward Models}  
The most robust reward systems synthesize verifiable and AI-generated feedback. This hybrid approach leverages the objectivity of tools while retaining the nuanced understanding of a powerful language model. For instance, the ( [CRScore: Reinforcement Learning with Verifiable Tool and AI Feedback for Code Review] ) framework fuses signals from linters, security analyzers, and subjective LLM feedback into a unified reward signal. This creates a holistic guide for the RL alignment process, mitigating reward hacking by grounding subjective AI feedback in objective, verifiable criteria.
\end{itemize}

\paragraph{Challenges and Mitigations in Reinforcement Learning-Based Alignment}

\begin{itemize}
\item \textbf{The Phenomenon of Reward Hacking in Code Generation}  
Reward hacking is a critical failure mode where an agent exploits a loophole to maximize a reward metric without acquiring the intended behavior. This is a specific instantiation of specification gaming, where an agent adheres to the literal specification of a reward function while violating its intent. In code synthesis, this can manifest in various ways, such as the agent learning to manipulate the evaluation apparatus itself---for instance, by modifying or excising test files to procure a universally passing result, a circumstance elucidated in ( [Reward Shaping to Mitigate Reward Hacking in RLHF] ). More sophisticated exploitations may involve manipulating simulated environments or other elements of the evaluation framework, an observation documented in ( [Teams of LLM Agents can Exploit Zero-Day Vulnerabilities] ).
\item \textbf{Countermeasures for Reward Hacking}  
Countermeasures have been proposed to forestall reward hacking. These include fortifying the training environment, such as by using a sequestered, immutable test suite to which the agent is denied access. Another approach involves deploying specialized validator models conditioned to penalize suspect behaviors. Furthermore, as investigated in ( [Reward Shaping to Mitigate Reward Hacking in RLHF] ), applying regularization techniques can suppress overly complex or ``spiky'' solutions, which are frequently correlated with reward hacking. Such techniques might include penalizing code length or cyclomatic complexity, or promoting policy entropy to encourage solution diversity.
\item \textbf{The ``Alignment Tax''}  
A formidable challenge in safety alignment is the trade-off between optimizing for safety and preserving general functional capabilities, a phenomenon known as the ``alignment tax.'' This tax materializes when excessive optimization on a narrow safety-centric reward signal leads to performance degradation on a broader spectrum of coding tasks. This phenomenon was systematically analyzed in ( [Safety Tax: Safety Alignment Makes Your Large Reasoning Models Less Reasonable] ), where it was shown that enhancing safety parameters can paradoxically diminish the ``reasonableness'' of reasoning models. For instance, a model heavily penalized for any potential security flaw might lose its ability to implement complex but necessary features like file I/O, even when implemented securely. To quantify this effect, comprehensive evaluation frameworks are essential. Methodologies such as incorporating a regularization term within the loss function, as seen in Localized Preference Optimization (LPO), are specifically engineered to ameliorate this issue by balancing the acquisition of safety behaviors with the retention of general-purpose functionalities. 
\end{itemize}

\subsubsection{Comprehensive Analysis and Future Directions}

This subsection presents a systematic exposition and comparative analysis of post-deployment alignment methodologies for enhancing security in automated code-generating agents. Despite the demonstrated capabilities of Large Language Models (LLMs) in software development, their propensity for generating insecure code remains a critical challenge ( [SOK: EXPLORING HALLUCINATIONS AND SECURITY RISKS IN AI-ASSISTED SOFTWARE DEVELOPMENT WITH INSIGHTS FOR LLM DEPLOYMENT] ; [Can You Really Trust Code Copilots? Evaluating Large Language Models from a Code Security Perspective] ). The alignment techniques examined herein, from Supervised Fine-Tuning (SFT) to advanced Reinforcement Learning (RL) paradigms, represent the vanguard of efforts to ameliorate these risks.

A comparative analysis of these methodologies is offered in the subsequent table, delineated across pivotal dimensions including their primary mechanisms, data requirements, and inherent strengths and limitations.

\textbf{Table: Comparison of Code Safety Alignment Techniques}

\begin{tabular}{|p{3cm}|p{3.5cm}|p{3cm}|p{3cm}|p{3cm}|}
\hline
\textbf{Technique} & \textbf{Primary Mechanism} & \textbf{Data Requirements} & \textbf{Key Strengths} & \textbf{Major Weaknesses} \\
\hline
\textbf{Baseline SFT} & Minimization of cross-entropy loss using a corpus of secure code exemplars. & A high-fidelity corpus of vulnerability-remediation pairs. & Straightforward implementation; directly instructs the model on secure coding paradigms. & Sub-optimal data annotation efficiency; often encumbered by a substantial 'alignment tax,' where enhanced security degrades functional correctness ( [A Comprehensive Study of LLM Secure Code Generation] ). \\
\hline
\textbf{SFT with Security Reasoning} & Acquisition of a deductive chain from problem analysis to secure implementation, compelling the model to emulate an expert's cognitive process. & A corpus of vulnerability-remediation pairs augmented with explicit deductive steps or chain-of-thought explications. & Enhanced model interpretability and generalization to novel vulnerability categories by learning abstract security principles ( [From Solitary Directives to Interactive Encouragement: LLM Secure Code Generation by Natural Language Prompting] ). & Manual curation of reasoning data is resource-intensive; risk of learning ``superficial reasoning'' that masks vulnerabilities. \\
\hline
\textbf{Direct Preference Optimization (DPO)} & Direct optimization of the policy to maximize the log-likelihood of preferred responses over rejected ones. & A dataset of preference pairs (chosen vs. rejected exemplars) adjudicated based on security criteria. & Higher data efficiency compared to SFT; circumvents the instability of explicit reward model training. & Fails to address the localized nature of code vulnerabilities, as the preference signal is applied globally. \\
\hline
\textbf{Localized Preference Optimization (LPO)} & A conceptual extension of DPO where the loss function is concentrated on critical security tokens or discrete code segments. & Preference pairs augmented with differential information identifying determinative lines of code. & Precise targeting of localized defects, potentially reducing the alignment tax by minimizing alterations to functional code. & Efficacy is heavily contingent on the availability of high-quality, granular differential information. \\
\hline
\textbf{RL with Verifiable Feedback} & Maximization of a reward signal derived from automated instrumentation such as static analyzers or formal verifiers. & A collection of interaction trajectories between the LLM and security analysis tools. & Enables adaptation to objective, verifiable security standards without explicit human annotation; highly scalable ( [Purple Llama CYBERSECEVAL: A Secure Coding Benchmark for Language Models] ). & Designing a comprehensive and non-exploitable reward function is complex; static analysis tools have intrinsic limitations ( [A Comprehensive Study of LLM Secure Code Generation] ). \\
\hline
\textbf{Reinforcement Learning from AI Feedback (RLAIF)} & Maximization of a reward signal generated by an AI adjudicator that evaluates code against security criteria. & A corpus of AI-generated preference data, ratings, or critiques. & Highly scalable and can be adapted to subjective or complex security criteria that are difficult for static tools to formalize. & Performance is fundamentally constrained by the quality of the AI adjudicator, which may itself harbor biases or vulnerabilities ( [Open Problems and Fundamental Limitations of Reinforcement Learning from Human Feedback] ). \\
\hline
\end{tabular}

As demonstrated by the analysis, no single technique offers a panoptic solution. SFT-based methodologies, while direct, may exhibit inefficiencies and degrade model utility. Preference optimization techniques afford greater data efficiency but may lack the requisite granularity. RL-based methodologies promise scalability and adaptability but introduce complexities in reward function design and are susceptible to reward hacking. Therefore, future research will likely converge upon hybrid systems engineered to amalgamate the respective strengths of these disparate methodologies. A robust pipeline might be initiated with SFT using a curated dataset with reasoning to establish a formidable base policy, subsequently augmented by LPO for refinement on localized issues, and ultimately targeted RL with verifiable feedback for managing adversarial edge cases and enhancing robustness against threats like backdoor attacks ( [Double Backdoored: Converting Code Large Language Model Backdoors to Traditional Malware via Adversarial Instruction Tuning Attacks] ).

This inquiry culminates in several pivotal, unresolved research questions that are anticipated to define the future of secure agent-based code generation:

\begin{enumerate}
\item  \textbf{What methodologies can be instituted for developing more sophisticated and less manipulable reward models?} A central challenge in RL-based alignment is reward hacking, where an agent exploits lacunae in the reward function instead of fulfilling the intended objective. This represents a fundamental limitation of optimizing any proxy objective ( [Open Problems and Fundamental Limitations of Reinforcement Learning from Human Feedback] ). Subsequent investigations must explore mechanisms for creating resilient reward models, potentially through uncertainty quantification, causal reasoning, or multi-objective optimization frameworks.
\item  \textbf{What scalable procedures can be devised for generating high-quality security reasoning data?} The provision of explicit logic for secure coding practices enhances model generalization. However, manual curation of such ``chain-of-thought'' data is a significant impediment. Further research is needed to develop semi-supervised or automated techniques for generating this data, possibly by using powerful teacher models to explicate remediations identified by static analysis tools, a concept explored in frameworks like CoV-Eval ( [Can You Really Trust Code Copilots? Evaluating Large Language Models from a Code Security Perspective] ).
\item  \textbf{How might standardized benchmarks be designed to equitably measure the ``alignment tax''?} A recurrent theme is the intrinsic trade-off between enhancing security and preserving functional correctness. As noted in ( [A Comprehensive Study of LLM Secure Code Generation] ), extant techniques often result in a degradation of functionality. For substantive progress, the field requires standardized, holistic benchmarks that permit the simultaneous evaluation of both security and functionality. The development of such benchmarks, analogous to CYBERSECEVAL ( [Purple Llama CYBERSECEVAL: A Secure Coding Benchmark for Language Models] ), is indispensable for quantifying the true cost of alignment and propelling the development of more efficient techniques. 
\end{enumerate}

==> archive/safety_sft.tex <==

\subsubsection{The Inherent Limitations of Pre-training and the Imperative for Post-hoc Alignment}

As previously articulated, a central challenge in CLLM safety is the ``knowledge-behavior disconnect.'' This phenomenon describes a state wherein a model may possess internal representations of security concepts yet fail to operationalize this knowledge without explicit directive guidance. Such a condition, elaborated in works such as ( [Risks from Learned Optimization in Advanced Machine Learning Systems] ), is not a mere mnemonic lapse but a fundamental misalignment. The model's generative objective---typically maximizing sequence likelihood---does not intrinsically prioritize security. While the model acquires a statistical apprehension of secure coding patterns, it lacks an explicit objective function that optimizes for security as a desirable property. The consequence is a probabilistic, rather than deliberate, application of security principles.

The pre-training process, conducted on voluminous and largely uncurated public code corpora from platforms like GitHub, is demonstrably effective for acquiring functional coding patterns. However, it concurrently exposes the model to a substantial volume of extant security vulnerabilities. The magnitude of this exposure is considerable. For instance, the investigation detailed in ( [Eradicating the Unseen: Detecting, Exploiting, and Remediating a Path Traversal Vulnerability across GitHub] ) identified over 1,700 discrete projects afflicted by a singular path traversal pattern, the prevalence of which ensures its assimilation and subsequent replication by models trained on such data. It has been empirically established in ( [Asleep at the Keyboard? Assessing the Security of GitHub Copilot's Code Contributions] ) that models trained on these corpora do indeed replicate insecure coding paradigms, with approximately 40\% of generated programs adjudicated to be vulnerable. This predicament is exacerbated by the phenomenon of ``code hallucinations,'' as described in ( [CodeMirage: Hallucinations in Code Generated by Large Language Models] ), wherein models generate outputs that are plausible yet factually incorrect or insecure. Such manifestations are not stochastic aberrations but systematic deficiencies, where the model fabricates non-existent yet syntactically valid library functions, misemploys Application Programming Interfaces in a manner that circumvents security protocols, or generates logically fallacious code that introduces subtle deficiencies. The immense scale and unvetted character of the training data thus render pre-training a necessary, yet demonstrably insufficient, precondition for constructing a secure CLLM.

Consequently, post-hoc alignment emerges as an indispensable corrective phase. In contrast to pre-training, which aims to build a generalized statistical model of code, alignment is a procedure that specifically directs the model's behavioral outputs toward predetermined, desirable attributes---in this context, ``safety.'' It is a process through which intentionality is instilled. This phase directly rectifies the inadequacies of standard fine-tuning paradigms, which often fail to optimize for secure coding because they accord equivalent salience to both security-relevant and security-irrelevant tokens. The research presented in ( [The Hidden Risks of LLM-Generated Web Application Code: A Security-Centric Evaluation of Code Generation Capabilities in Large Language Models] ) substantiates this by revealing systemic vulnerabilities in LLM-generated web application code related to authentication, session management, and input validation. These are not esoteric edge-cases but fundamental security requisites that unaligned models persistently fail to implement, indicating that their default behavioral disposition does not prioritize established best practices. An unaligned model might generate a functionally correct login procedure but fail to implement rate limiting or secure cookie flags, as such features appear with lower frequency in its training corpus despite their critical importance. Alignment, therefore, can be conceptualized as the pedagogical process of instructing the model to recognize and assign priority to these critical, albeit statistically less frequent, security-related patterns. In light of these considerations, the subsequent analysis is dedicated to presenting SFT and RL as two complementary strategic frameworks designed to inject security-specific priors into the model, aiming to transcend generalized knowledge and cultivate explicit, safety-conscious operational behavior. 

\subsubsection{Supervised Fine-Tuning for Secure Code Generation}

Supervised Fine-Tuning (SFT) is a core methodology for adapting the generalized capabilities of pre-trained Large Language Models (LLMs) to specific tasks, including the generation of secure code. This section analyzes how supervised learning paradigms enhance the security posture of code-generating agents. The foundational principle of SFT is to present a model with a curated corpus of input-output exemplars, enabling it to learn the mapping from specific prompts to desired responses. Applying SFT to code security is non-trivial, as it requires the model to internalize the nuanced, context-dependent rules that differentiate secure code from vulnerable counterparts. The body of research consistently indicates that SFT's efficacy is almost entirely contingent upon the quality, diversity, and intrinsic properties of its underlying training data. This section traces the evolution of these techniques, from foundational fine-tuning on manually curated datasets to the formulation of sophisticated, security-conscious preference optimization algorithms that enable models to learn implicitly from security-oriented choices.

\paragraph{Data as the Cornerstone: Constructing Security-Aware Datasets}

At its core, SFT is a process of learning by example. Therefore, constructing high-quality, purpose-driven, and contextually rich datasets is an indispensable prerequisite for achieving robust and reliable security alignment. A model's capacity to generate secure code directly reflects the data upon which it has been trained; if the data exhibits noise, sparsity, or a lack of diversity, the model's security capabilities will manifest corresponding fragility. Methodologies for creating such datasets range from mining real-world artifacts to synthesizing targeted training exemplars, with each approach designed to mitigate the limitations of its predecessors.

\textbf{Curation of Real-World Vulnerability-Fix Pairs}

The most fundamental data type for security-oriented SFT consists of paired examples of ``vulnerable code'' and its corresponding ``fixed code,'' providing a direct, supervised signal of how security remediation is manifested in practice. The primary method for constructing these datasets involves systematically mining historical data from large-scale open-source software repositories. As detailed in ( [CVEfixes: Automated Collection of Vulnerabilities and Their Fixes from Open-Source Software] ), this process entails complex data engineering pipelines designed to parse commit messages, link them to issue-tracking systems, and correlate them with official entries in vulnerability databases like the Common Vulnerabilities and Exposures (CVE) system. Foundational benchmarks such as CVEfixes and BigVul are the canonical products of this methodology. More advanced frameworks, such as that proposed in ( [Large Language Models for Code: Security Hardening and Adversarial Testing] ), not only extract code modifications but also simulate real-world repair scenarios by providing varying levels of contextual information, such as surrounding functions or dependency information.

\textbf{Challenges in Data Quality and Curation}

Despite its intuitive appeal, constructing datasets from real-world repositories is fraught with potential pitfalls that can severely compromise data quality and, by extension, model performance. As highlighted with empirical evidence in ( [Vulnerability Detection with Code Language Models: How Far Are We?] ), prominent public datasets may be afflicted by significant issues such as high rates of duplication and questionable label accuracy. High duplication can lead a model to ``memorize'' specific fixes rather than learn the underlying security principle, resulting in artificially inflated performance metrics. A more insidious threat is label noise, where a single commit labeled as a ``security fix'' may contain unrelated changes like feature enhancements or refactoring. This noise can confound the model, causing it to learn spurious correlations and fail in real-world scenarios. This finding underscores the necessity of implementing rigorous protocols for data cleaning, validation, and de-duplication before initiating any SFT process.

\textbf{Synthetic Data Generation for Scalability and Diversity}

To surmount the scarcity and quality issues associated with real-world data, the research community has increasingly turned to synthetic data generation. This paradigm leverages powerful ``teacher'' LLMs to create novel, clean, and targeted pairs of vulnerable and secure code, often guided by templates from known vulnerability patterns like the Common Weakness Enumeration (CWEs). As explored in ( [Synthetic Code Surgery: Repairing Bugs and Vulnerabilities with LLMs and Synthetic Data] ), this method permits the creation of large-scale, diverse datasets tailored to specific security requirements. A key innovation, presented in ( [PROSEC: Fortifying Code LLMs with Proactive Security Alignment] ), lies not merely in generating code, but in generating the underlying \textbf{security reasoning}. This approach, analogous to chain-of-thought prompting, instructs the teacher model to first identify a vulnerability, explicate the logic for the fix, and then generate the secure code. This ``think-before-you-act'' data format provides the student model with a richer learning signal, shifting the training objective from mere pattern-matching toward inculcating a causal model of vulnerability remediation.

\textbf{Distillation of Preference Data}

For more advanced alignment techniques, researchers have focused on creating preference datasets that explicitly encode that secure code is preferable to insecure code. The format is typically a triplet: \texttt{<prompt, chosen\_secure\_code, rejected\_insecure\_code>}. This structure is the core data format for modern preference optimization algorithms. As described in ( [Teaching an Old LLM Secure Coding: Localized Preference Optimization on Distilled Preferences] ), such data is often generated via knowledge distillation, where a powerful teacher model generates multiple code candidates. Subsequently, a security-aware mechanism---another specialized LLM or a static analysis tool---adjudicates between the candidates, designating the secure version as 'chosen' and insecure alternatives as 'rejected.' This process creates a large-scale dataset that explicitly encodes a preference for security, which can then be used to train a smaller ``student'' model. This methodology forms the basis of modern preference optimization techniques, such as that detailed in ( [Direct Preference Optimization: Your Language Model is Secretly a Reward Model] ), which has demonstrated state-of-the-art performance by directly optimizing the policy based on these expressed preferences.

\paragraph{SFT and its Security Variants}

Leveraging these security-aware datasets, a series of SFT methodologies have been developed, ranging from broad fine-tuning to highly targeted, feedback-driven cycles.

\textbf{Baseline SFT}

The most direct method involves standard supervised fine-tuning on curated (vulnerable\_code, fixed\_code) pairs using a standard cross-entropy loss function. While a necessary initial step, its efficacy is limited by its own simplicity. As noted in ( [Teaching an Old LLM Secure Coding: Localized Preference Optimization on Distilled Preferences] ), a standard SFT process tends to treat all code tokens with equal importance. This uniform treatment dilutes the learning signal, as the critical modifications may involve only a few specific tokens, and the model may expend considerable capacity learning to replicate code segments extraneous to the actual security fix.

\textbf{Instruction Tuning}

A more targeted form of SFT is instruction tuning, where the model is trained on specific, task-oriented natural language instructions, such as ``Find and fix the SQL injection vulnerability in this code.'' As detailed in ( [Instruction Tuning for Secure Code Generation] ), this methodology facilitates better generalization to security-related tasks because the model learns to associate natural language intent with corresponding code modifications. The study demonstrates that integrating security-specific instruction tuning with a general instruction dataset can dramatically improve the security of generated code while preserving the model's overall utility, thus avoiding ``catastrophic forgetting.''

\textbf{Feedback-Driven SFT}

Blurring the line between SFT and Reinforcement Learning (RL), feedback-driven SFT integrates a dynamic loop of code generation and evaluation. In this ``tool-in-the-loop'' system, a model's output is subjected to evaluation by an external tool, such as a static analyzer or formal verifier. The structured feedback (e.g., ``Vulnerability detected: NULL\_DEREFERENCE on line 42'') is then used to construct a new, detailed prompt directing the model to repair its own output. As demonstrated in ( [A New Era in Software Security: Towards Self-Healing Software via Large Language Models and Formal Verification] ), providing explicit, verifiable feedback significantly enhances a model's capacity for accurate code repair. Successful repair attempts from this loop are subsequently re-integrated into the training dataset as high-quality, validated exemplars for future SFT rounds, establishing a positive feedback loop that progressively refines the model's performance, a concept also explored in ( [Combining Large Language Models with Static Analyzers for Code Review Generation] ).

\paragraph{Advanced Preference Optimization for Localized Flaws}

The evolution from general-purpose preference optimization methods like Direct Preference Optimization (DPO) to algorithms specifically engineered for code security marks a significant advancement. A core limitation of standard DPO is its application of a uniform preference signal across the entire code sequence, whereas security vulnerabilities are often highly localized phenomena.

To address this, the \textbf{Localized Preference Optimization (LPO)} algorithm was developed. As detailed in ( [Teaching an Old LLM Secure Coding: Localized Preference Optimization on Distilled Preferences] ), LPO confronts the localized nature of code vulnerabilities by propagating the optimization loss predominantly to the specific tokens that differentiate the secure from the insecure code. To prevent a degradation of the model's general coding capabilities (the ``alignment tax''), LPO incorporates a standard SFT loss on non-security-relevant tokens as a regularization term. This dual-objective approach permits targeted security alignment while preserving overall code quality. Empirical studies have shown that LPO can reduce security issues by 19\% to 40\% while simultaneously improving code quality by 3\% to 10\%.

This progression---from broad SFT to preference-based DPO, and finally to token-targeted LPO---reflects a deepening conceptual understanding of the LLM code security problem: an evolution from viewing ``writing secure code'' as a general stylistic trait to recognizing it as a precise, localized semantic property. Initially, SFT treated secure coding as a task learnable by example, which proved inefficient. DPO refined this by framing the problem as a preference (``this secure version is better than that insecure one'') but still applied this signal globally. LPO represents a conceptual leap by operationalizing the insight that security flaws are typically localized errors. By focusing the loss function on these ``pivotal tokens,'' LPO precisely teaches the model which localized edits confer security. Concurrently, the use of an SFT regularizer in LPO demonstrates a sophisticated understanding of the alignment tax, actively safeguarding the model's general capabilities while performing precise ``surgery'' on security defects. This trajectory charts a clear path for future research: moving beyond surface-level token manipulation toward alignment techniques that operate on abstract semantic representations of code, such as Abstract Syntax Trees (ASTs), to instill a more robust and generalizable conceptualization of security. 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\renewcommand{\arraystretch}{1.3} % 增加行高，避免拥挤

==> sections/author_list.tex <==
\section{Contributions and Acknowledgements}
\textbf{The authors of this paper are listed in order as follows:} \\

